ImagenHub: Standardizing the evaluation of conditional image generation models

Recently, a myriad of conditional image generation and editing models have been developed to serve different downstream tasks, including text-to-image generation, text-guided image editing, subject-driven image generation, control-guided image generation, etc. However, we observe huge inconsistencies in experimental conditions: datasets, inference, and evaluation metrics - render fair comparisons difficult. This paper proposes ImagenHub, which is a one-stop library to standardize the inference and evaluation of all the conditional image generation models. Firstly, we define seven prominent tasks and curate high-quality evaluation datasets for them. Secondly, we built a unified inference pipeline to ensure fair comparison. Thirdly, we design two human evaluation scores, i.e. Semantic Consistency and Perceptual Quality, along with comprehensive guidelines to evaluate generated images. We train expert raters to evaluate the model outputs based on the proposed metrics. Our human evaluation achieves a high inter-worker agreement of Krippendorff's alpha on 76% models with a value higher than 0.4. We comprehensively evaluated a total of around 30 models and observed three key takeaways: (1) the existing models' performance is generally unsatisfying except for Text-guided Image Generation and Subject-driven Image Generation, with 74% models achieving an overall score lower than 0.5. (2) we examined the claims from published papers and found 83% of them hold with a few exceptions. (3) None of the existing automatic metrics has a Spearman's correlation higher than 0.2 except subject-driven image generation. Moving forward, we will continue our efforts to evaluate newly published models and update our leaderboard to keep track of the progress in conditional image generation.

==> sections/backup.tex <==
\subsection{Detailed human evaluation results}

\begin{table}[!t]
\centering
\small
\begin{tabular}{l|cc|cc|cc}
\toprule
Model & $SC_{Avg}$ & $\text{Kappa}_{SC}$ &  $PQ_{Avg}$ & $\text{Kappa}_{PQ}$ & $\text{Overall}$ & $\text{Kappa}_{\bar{O}}$ \\
\midrule
\multicolumn{7}{c}{Text-to-Image Generation} \\
\midrule
DeepFloydIF & 0.65$\pm$0.02 & 0.53 & 0.62$\pm$0.06 & 0.21 & \textbf{0.59$\pm$0.02} & 0.32\\
Stable Diffusion XL & 0.62$\pm$0.03 & 0.49 & 0.64$\pm$0.05 & 0.36 & 0.59$\pm$0.03 & 0.37\\
Dalle-2 & 0.58$\pm$0.04 & 0.37 & 0.62$\pm$0.06 & 0.39 & 0.54$\pm$0.04 & 0.27\\
OpenJourney & 0.53$\pm$0.02 & 0.46 & 0.59$\pm$0.05 & 0.24 & 0.50$\pm$0.02 & 0.30\\
Stable Diffusion 2.1 & 0.56$\pm$0.02 & 0.55 & 0.53$\pm$0.05 & 0.23 & 0.50$\pm$0.03 & 0.38\\
\midrule
\multicolumn{7}{c}{Mask-guided Image Editing} \\
\midrule
SDXL-Inpainting & 0.49$\pm$0.05 & 0.58 & 0.51$\pm$0.02 & 0.42  & \textbf{0.37$\pm$0.05} & 0.50\\
SD-Inpainting & 0.28$\pm$0.04 & 0.55 & 0.27$\pm$0.10 & 0.26  & 0.17$\pm$0.07 & 0.31\\
GLIDE & 0.20$\pm$0.05 & 0.46 & 0.48$\pm$0.06 & 0.28  & 0.16$\pm$0.05 & 0.33\\
BlendedDiffusion & 0.12$\pm$0.03 & 0.44 & 0.11$\pm$0.03 & 0.45  & 0.05$\pm$0.02 & 0.36\\
\midrule
\multicolumn{7}{c}{Text-guided Image Editing} \\
\midrule
MagicBrush        & 0.51$\pm$0.01  & 0.50 & 0.65$\pm$0.06 & 0.35  & \textbf{0.47$\pm$0.02} & 0.44\\
InstructPix2Pix   & 0.29$\pm$0.01  & 0.60 & 0.70$\pm$0.06 & 0.41  & 0.27$\pm$0.02 & 0.55\\
Prompt-to-prompt  & 0.17$\pm$0.05  & 0.42 & 0.55$\pm$0.09 & 0.33  & 0.15$\pm$0.06 & 0.36\\
CycleDiffusion    & 0.17$\pm$0.03  & 0.46 & 0.56$\pm$0.11 & 0.38  & 0.14$\pm$0.04 & 0.41\\
SDEdit            & 0.04$\pm$0.03  & 0.20 & 0.56$\pm$0.12 & 0.23  & 0.04$\pm$0.03 & 0.13\\
Text2Live         & 0.02$\pm$0.01  & 0.24 & 0.82$\pm$0.04 & 0.39  & 0.02$\pm$0.02 & 0.10\\
DiffEdit          & 0.02$\pm$0.01  & 0.18 & 0.23$\pm$0.04 & 0.56  & 0.01$\pm$0.01 & 0.24\\
Pix2PixZero       & 0.01$\pm$0.00  & 0.37 & 0.48$\pm$0.09 & 0.43  & 0.01$\pm$0.01 & 0.37\\
\midrule
\multicolumn{7}{c}{Subject-driven Image Generation} \\
\midrule
SuTI              & 0.64$\pm$0.11 & 0.30 & 0.68$\pm$0.08 & 0.24 & \textbf{0.58$\pm$0.12} & 0.20\\
DreamBooth        & 0.51$\pm$0.08 & 0.40 & 0.93$\pm$0.02 & 0.39 & 0.55$\pm$0.11 & 0.37\\
BLIP-Diffusion    & 0.29$\pm$0.04 & 0.23 & 0.93$\pm$0.04 & 0.12 & 0.35$\pm$0.06 & 0.22\\
TextualInversion  & 0.21$\pm$0.04 & 0.43 & 0.74$\pm$0.08 & 0.24 & 0.21$\pm$0.05 & 0.35\\
DreamBooth-Lora   & 0.07$\pm$0.01 & 0.30 & 0.82$\pm$0.07 & 0.36 & 0.09$\pm$0.01 & 0.29\\
\midrule
\multicolumn{7}{c}{Multi-concept Image Composition} \\
\midrule
CustomDiffusion   & 0.26$\pm$0.01 & 0.83 & 0.86$\pm$0.05 & 0.41  & \textbf{0.29$\pm$0.01} & 0.73\\
DreamBooth        & 0.11$\pm$0.02 & 0.65 & 0.78$\pm$0.02 & 0.69  & 0.13$\pm$0.02 & 0.61\\
TextualInversion  & 0.04$\pm$0.01 & 0.73 & 0.74$\pm$0.05 & 0.54  & 0.05$\pm$0.01 & 0.62\\
\midrule
\multicolumn{7}{c}{Subject-driven Image Editing} \\
\midrule
PhotoSwap         & 0.34$\pm$0.02 & 0.33 & 0.65$\pm$0.04 & 0.15  & \textbf{0.36$\pm$0.02} & 0.35\\
DreamEdit         & 0.31$\pm$0.03 & 0.45 & 0.61$\pm$0.03 & 0.13  & 0.32$\pm$0.03 & 0.33\\
BLIP-Diffusion    & 0.09$\pm$0.03 & 0.44 & 0.70$\pm$0.02 & 0.26  & 0.09$\pm$0.03 & 0.41\\
\midrule
\multicolumn{7}{c}{Control-guided Image Generation} \\
\midrule
ControlNet        & 0.42$\pm$0.05 & 0.42 & 0.19$\pm$0.04 & 0.41  & \textbf{0.23$\pm$0.04} & 0.37\\
UniControl        & 0.38$\pm$0.07 & 0.45 & 0.20$\pm$0.06 & 0.42  & 0.23$\pm$0.07 & 0.36\\
\bottomrule
\end{tabular}
\caption{All the evaluated models from seven core tasks. }
\label{tab:result}
\end{table}


\begin{table}[!ht]
\small
\centering
\begin{tabular}{@{}lcc@{}}
\toprule
Task & Data Source & Inference Dataset size \\ \midrule
Text-guided Image Generation & \begin{tabular}[c]{@{}c@{}}DrawBench~\citep{saharia2022photorealistic} \\ DiffusionDB~\citep{wangDiffusionDBLargescalePrompt2022} \\ ABC-6K~\citep{feng2023trainingfree}\\ Ours\end{tabular} & 197 \\ \midrule
Mask-guided Image Editing & \begin{tabular}[c]{@{}c@{}}MagicBrush~\citep{zhang2023magicbrush} \\ Ours\end{tabular} & 179 \\ \midrule
Text-guided Image Editing & \begin{tabular}[c]{@{}c@{}}MagicBrush~\citep{zhang2023magicbrush} \\ Ours\end{tabular} & 179 \\ \midrule
Subject-driven Image Generation & \begin{tabular}[c]{@{}c@{}}SuTI~\citep{chen2023subject} \\ Ours\end{tabular} & 150 \\ \midrule
Multi-concept Image Composition & \begin{tabular}[c]{@{}c@{}}CustomDiffsion~\citep{kumari2023multi} \\ Ours\end{tabular} & 102 \\ \midrule
Subject-driven Image Editing & DreamEditBench~\citep{li2023dreamedit} & 154 \\ \midrule
Control-guided Image Generation & HuggingFace community & 150 \\ \bottomrule
\end{tabular}
\caption{All the human evaluation datasets from seven core tasks. }
\label{tab:dataset}
\end{table}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/task_performance.png}
    \caption{Model performance in each task.}
    \label{fig:performance_all_tasks}
\end{figure}

\begin{table*}[htb]
% \parbox{.3\linewidth}{
\begin{minipage}{.4\linewidth}
\resizebox{\columnwidth}{!}{%    
\begin{tabular}{l|cc|cc|cc}
\toprule
\multirow{2}{*}{Setting} &  \multicolumn{2}{c|}{$\sqrt{SC \times PQ}$} & \multicolumn{2}{c|}{$\alpha_1SC + \beta_1PQ$} & \multicolumn{2}{c}{$\alpha_2SC + \beta_2PQ$}\\
   & $O_{Sum}$   & $O_{Avg}$  & $O_{Sum}$   & $O_{Avg}$  &$O_{Sum}$   & $O_{Avg}$  \\
\midrule
MagicBrush &  83.51 & 0.47   & 103.75  &  0.58 & 98.85 & 0.55 \\
CycleDiffusion   &  24.89 & 0.14   & 65.25  &  0.36 & 51.28 & 0.29 \\
DiffEdit   &  1.71 & 0.01   & 22.08  &  0.12 & 14.38 & 0.08 \\
Text2Live   &  4.08 & 0.02   & 75.25  &  0.42 & 46.75 & 0.26 \\
\bottomrule
\end{tabular}
}
    \label{tab:i2t_bridge}
% 	\vspace{-2ex}
% }
\end{minipage} 
% \hfill
\hspace{4pt}
% \parbox{.3\linewidth}{
\begin{minipage}{.6\linewidth}
\resizebox{\columnwidth}{!}{%    
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
\multirow{2}{*}{Setting} &  \multicolumn{3}{c|}{[0, 0.5, 1]} & \multicolumn{3}{c|}{[0, 0.5, 1, 2]} & \multicolumn{3}{c}{[0, 1]}\\
& $O_{Avg}$ & $\text{Fleiss}_{\bar{O}}$   & $\text{Kd}_{\bar{O}}$ & $O_{Avg}$ & $\text{Fleiss}_{\bar{O}}$   & $\text{Kd}_{\bar{O}}$  & $O_{Avg}$ & $\text{Fleiss}_{\bar{O}}$ & $\text{Kd}_{\bar{O}}$  \\
\midrule
BLIP-Diffusion  & 0.13 &  0.41 & 0.47   & 0.09 & 0.29  & 0.50  & 0.05 &  0.40 & 0.40   \\
DreamEdit  & 0.50 &  0.33 & 0.52   & 0.32 & 0.26  &  0.55 & 0.21 & 0.38 & 0.38  \\
PhotoSwap  & 0.62 &  0.35 & 0.46   & 0.36 & 0.25  &  0.50 & 0.29 & 0.37 & 0.37   \\
\bottomrule
\end{tabular}
}

    \label{tab:t2i_bridge}
\end{minipage} 
\end{table*}

\begin{tabularx}{\textwidth}{*{2}{>{\centering\arraybackslash}X}}
   \small
   \centering
\includegraphics[width=0.9\linewidth,valign=m]{figures/task_performance.pdf} % <-- valing is chanded from T to m
&
    \begin{tabular}{@{}cc@{}}
    \toprule
    Data Source & Size \\ 
    \midrule
    \begin{tabular}[c]{@{}c@{}}\textcolor{Green}{DrawBench~\citep{saharia2022photorealistic}} \\ \textcolor{Green}{DiffusionDB~\citep{wangDiffusionDBLargescalePrompt2022}} \\ \textcolor{Green}{ABC-6K~\citep{feng2023trainingfree}}\\ \textcolor{Green}{Ours}\end{tabular} & \textcolor{Green}{197} \\ 
    \midrule
    \begin{tabular}[c]{@{}c@{}}\textcolor{Brown}{MagicBrush~\citep{zhang2023magicbrush}} \\ \textcolor{Brown}{Ours}\end{tabular} & \textcolor{Brown}{179} \\ 
    \midrule
    \begin{tabular}[c]{@{}c@{}}\textcolor{Purple}{MagicBrush~\citep{zhang2023magicbrush}} \\ \textcolor{Purple}{Ours}\end{tabular} & \textcolor{Purple}{179} \\ 
    \midrule
    \begin{tabular}[c]{@{}c@{}}\textcolor{Orange}{SuTI~\citep{chen2023subject}} \\ \textcolor{Orange}{Ours}\end{tabular} & \textcolor{Orange}{150} \\
    \midrule
    \begin{tabular}[c]{@{}c@{}}\textcolor{Cyan}{CustomDiffsion~\citep{kumari2023multi}} \\ \textcolor{Cyan}{Ours}\end{tabular} & \textcolor{Cyan}{102} \\ 
    \midrule
    \textcolor{NavyBlue}{DreamEditBench~\citep{li2023dreamedit}} & \textcolor{NavyBlue}{154} \\ 
    \midrule
    \textcolor{BrickRed}{HuggingFace community} & \textcolor{BrickRed}{150} \\ \bottomrule
    \end{tabular}
\captionof{table}{Task Dataset Statistics}
\label{tab:dataset}
&   \vspace{-0.7cm}
    \captionof{figure}{Task Performance Distribution}
    \label{fig:performance_all_tasks}
    \vspace{-2ex}
\end{tabularx}




\begin{table}[H]
\centering
\small
\scalebox{0.95}{
\begin{tabular}{l|cccc|c}
\toprule
Model & LPIPS ↓ &  DINO ↑ & CLIP-I ↑ & DreamSim ↓ & CLIP ↑\\
\midrule
\multicolumn{6}{c}{Text-guided Image Generation} \\
\midrule
DeepFloydIF         & N/A & N/A & N/A & N/A & 0.2814 \\
Stable Diffusion XL & N/A & N/A & N/A & N/A & 0.2886 \\
Dalle-2             & N/A & N/A & N/A & N/A & 0.2712 \\
OpenJourney         & N/A & N/A & N/A & N/A & 0.2814 \\
Stable Diffusion    & N/A & N/A & N/A & N/A & 0.2899 \\
\midrule
\multicolumn{6}{c}{Mask-guided Image Editing} \\
\midrule
SDXL-Inpainting  & 0.15 & 0.90 & 0.94 & 0.15 & 0.2729 \\
SD-Inpainting    & 0.21 & 0.85 & 0.91 & 0.20 & 0.2676 \\
GLIDE            & 0.18 & 0.91 & 0.94 & 0.14 & 0.2578 \\
BlendedDiffusion & 0.33 & 0.80 & 0.87 & 0.26 & 0.2594 \\
\midrule
\multicolumn{6}{c}{Text-guided Image Editing} \\
\midrule
MagicBrush        & 0.22 & 0.88 & 0.92 & 0.19 & 0.2675 \\
InstructPix2Pix   & 0.32 & 0.77 & 0.86 & 0.30 & 0.2616 \\
Prompt-to-prompt  & 0.40 & 0.68 & 0.81 & 0.36 & 0.2674 \\
CycleDiffusion    & 0.28 & 0.79 & 0.88 & 0.27 & 0.2692 \\
SDEdit            & 0.61 & 0.57 & 0.76 & 0.50 & 0.2872 \\
Text2Live         & 0.17 & 0.87 & 0.92 & 0.18 & 0.2628 \\
DiffEdit          & 0.22 & 0.78 & 0.85 & 0.31 & 0.2425 \\
Pix2PixZero       & 0.60 & 0.53 & 0.76 & 0.52 & 0.2510 \\
\midrule
\multicolumn{6}{c}{Subject-driven Image Generation} \\
\midrule
SuTI              & 0.77 & 0.69 & 0.81 & 0.32 & 0.2895 \\
DreamBooth        & 0.77 & 0.61 & 0.80 & 0.40 & 0.2847 \\
BLIP-Diffusion    & 0.77 & 0.63 & 0.82 & 0.36 & 0.2729 \\
TextualInversion  & 0.81 & 0.37 & 0.65 & 0.61 & 0.2680 \\
DreamBooth-Lora   & 0.82 & 0.36 & 0.70 & 0.61 & 0.2988 \\
\midrule
\multicolumn{6}{c}{Subject-driven Image Editing} \\
\midrule
PhotoSwap         & 0.34 & 0.65 & 0.83 & 0.37 & 0.2846 \\
DreamEdit         & 0.22 & 0.74 & 0.87 & 0.28 & 0.2855 \\
BLIP-Diffusion    & 0.25 & 0.80 & 0.89 & 0.23 & 0.2901 \\
\midrule
\multicolumn{6}{c}{Multi-concept Image Composition} \\
\midrule
CustomDiffusion   & 0.79 & 0.50 & 0.70 & 0.55 & 0.2929 \\
DreamBooth        & 0.78 & 0.39 & 0.64 & 0.66 & 0.2993 \\
TextualInversion  & 0.80 & 0.44 & 0.66 & 0.65 & 0.2548 \\
\midrule
\multicolumn{6}{c}{Control-guided Image Generation} \\
\midrule
ControlNet        & 0.80 & 0.43 & 0.70  & 0.56 & 0.2555 \\
UniControl        & 0.82 & 0.42 & 0.68 & 0.58 & 0.2604 \\
\bottomrule
\end{tabular}}
\caption{All automated metrics for the evaluated models.}
\label{tab:metrics_extra}
\end{table}


\section{Datasheet}

\subsection{Continuous update of Human evaluation score}

\begin{table}[H]
\centering
\scalebox{0.85}{
\begin{tabular}{l|cc|c|cc}
\toprule
Model & $SC_{Avg}$ &  $PQ_{Avg}$ & $\text{Overall}$ & $\text{Fleiss}_{\bar{O}}$ & $\text{Kd}_{\bar{O}}$\\
\midrule
\multicolumn{6}{c}{Text-guided Image Generation} \\
\midrule
Dalle-3 & 0.79$\pm$0.02 & 0.79$\pm$0.14 & \textbf{0.76$\pm$0.08} & 0.19 & 0.34\\
Midjourney & 0.67$\pm$0.06 & 0.92$\pm$0.06 & 0.73$\pm$0.07 & 0.34 & 0.51\\

DeepFloydIF & 0.65$\pm$0.02 & 0.62$\pm$0.06 & 0.59$\pm$0.02 & 0.32 & 0.51\\
Stable Diffusion XL & 0.62$\pm$0.03 & 0.64$\pm$0.05 & 0.59$\pm$0.03 & 0.37 & 0.61\\
Dalle-2 & 0.58$\pm$0.04 & 0.62$\pm$0.06 & 0.54$\pm$0.04 & 0.27 & 0.40\\
OpenJourney & 0.53$\pm$0.02 & 0.59$\pm$0.05 & 0.50$\pm$0.02 & 0.30 & 0.47\\
Stable Diffusion 2.1 & 0.56$\pm$0.02 & 0.53$\pm$0.05 & 0.50$\pm$0.03 & 0.38 & 0.50\\
\midrule
\multicolumn{6}{c}{Mask-guided Image Editing} \\
\midrule
SDXL-Inpainting & 0.49$\pm$0.05 & 0.51$\pm$0.02 & \textbf{0.37$\pm$0.05} & 0.50 & 0.72\\
SD-Inpainting & 0.28$\pm$0.04 & 0.27$\pm$0.10 & 0.17$\pm$0.07 & 0.31 & 0.49\\
GLIDE & 0.20$\pm$0.05 & 0.48$\pm$0.06 & 0.16$\pm$0.05 & 0.33 & 0.56 \\
BlendedDiffusion & 0.12$\pm$0.03 & 0.11$\pm$0.03 & 0.05$\pm$0.02 & 0.36 & 0.44\\
\midrule
\multicolumn{6}{c}{Text-guided Image Editing} \\
\midrule
MagicBrush        & 0.51$\pm$0.01  & 0.65$\pm$0.06 & \textbf{0.47$\pm$0.02} & 0.44 & 0.67\\
InstructPix2Pix   & 0.29$\pm$0.01  & 0.70$\pm$0.06 & 0.27$\pm$0.02 & 0.55 & 0.74\\
Prompt-to-prompt  & 0.17$\pm$0.05  & 0.55$\pm$0.09 & 0.15$\pm$0.06 & 0.36 & 0.53\\
CycleDiffusion    & 0.17$\pm$0.03  & 0.56$\pm$0.11 & 0.14$\pm$0.04 & 0.41 & 0.63\\
SDEdit            & 0.04$\pm$0.03  & 0.56$\pm$0.12 & 0.04$\pm$0.03 & 0.13 & 0.13\\
Text2Live         & 0.02$\pm$0.01  & 0.82$\pm$0.04 & 0.02$\pm$0.02 & 0.10 & 0.17\\
DiffEdit          & 0.02$\pm$0.01  & 0.23$\pm$0.04 & 0.01$\pm$0.01 & 0.24 & 0.24\\
Pix2PixZero       & 0.01$\pm$0.00  & 0.48$\pm$0.09 & 0.01$\pm$0.01 & 0.37 & 0.37\\
\midrule
\multicolumn{6}{c}{Subject-driven Image Generation} \\
\midrule
SuTI              & 0.64$\pm$0.11 & 0.68$\pm$0.08 & \textbf{0.58$\pm$0.12} & 0.20 & 0.39\\
DreamBooth        & 0.51$\pm$0.08 & 0.93$\pm$0.02 & 0.55$\pm$0.11 & 0.37 & 0.60\\
BLIP-Diffusion    & 0.29$\pm$0.04 & 0.93$\pm$0.04 & 0.35$\pm$0.06 & 0.22 & 0.39\\
TextualInversion  & 0.21$\pm$0.04 & 0.74$\pm$0.08 & 0.21$\pm$0.05 & 0.35 & 0.52\\
DreamBooth-Lora   & 0.07$\pm$0.01 & 0.82$\pm$0.07 & 0.09$\pm$0.01 & 0.29 & 0.37\\
\midrule
\multicolumn{6}{c}{Subject-driven Image Editing} \\
\midrule
PhotoSwap         & 0.34$\pm$0.02 & 0.65$\pm$0.04 & \textbf{0.36$\pm$0.02} & 0.35 & 0.46\\
DreamEdit         & 0.31$\pm$0.03 & 0.61$\pm$0.03 & 0.32$\pm$0.03 & 0.33 & 0.52\\
BLIP-Diffusion    & 0.09$\pm$0.03 & 0.70$\pm$0.02 & 0.09$\pm$0.03 & 0.41 & 0.47\\
\midrule
\multicolumn{6}{c}{Multi-concept Image Composition} \\
\midrule
CustomDiffusion   & 0.26$\pm$0.01 & 0.86$\pm$0.05 & \textbf{0.29$\pm$0.01} & 0.73 & 0.88\\
DreamBooth        & 0.11$\pm$0.02 & 0.78$\pm$0.02 & 0.13$\pm$0.02 & 0.61 & 0.71\\
TextualInversion  & 0.04$\pm$0.01 & 0.74$\pm$0.05 & 0.05$\pm$0.01 & 0.62 & 0.77\\
\midrule
\multicolumn{6}{c}{Control-guided Image Generation} \\
\midrule
ControlNet        & 0.42$\pm$0.05 & 0.19$\pm$0.04 & \textbf{0.23$\pm$0.04} & 0.37 & 0.57\\
UniControl        & 0.38$\pm$0.07 & 0.20$\pm$0.06 & 0.23$\pm$0.07 & 0.36 & 0.58\\
\bottomrule
\end{tabular} }
\caption{Updated table with extra models.}
\label{tab:result_extra}
\end{table}


